Gaia DR3 astrometric orbit determination with Markov Chain Monte Carlo and Genetic Algorithms. Systems with stellar, substellar, and planetary mass companions

Astrometric discovery of sub-stellar mass companions orbiting stars is exceedingly hard due to the required sub-milliarcsecond precision, limiting the application of this technique to only a few instruments on a target-per-target basis as well as the global astrometry space missions Hipparcos and Gaia. The third Gaia data release includes the first Gaia astrometric orbital solutions, whose sensitivity in terms of estimated companion mass extends down into the planetary-mass regime. We present the contribution of the `exoplanet pipeline' to the Gaia DR3 sample of astrometric orbital solutions by describing the methods used for fitting the orbits, the identification of significant solutions, and their validation. We then present an overview of the statistical properties of the solution parameters. Using both a Markov Chain Monte Carlo and Genetic Algorithm we fit the 34 months of Gaia DR3 astrometric time series with a single Keplerian astrometric-orbit model. Verification and validation steps are taken using significance tests, internal consistency checks using the Gaia radial velocity measurements (when available), as well as literature radial velocity and astrometric data, leading to a subset of candidates that are labelled as 'validated'. We determined astrometric-orbit solutions for 1162 sources and 198 solutions have been assigned the 'validated' label. Precise companion mass estimates are presented elsewhere. From internal and external verification and validation we estimate the level of spurious/incorrect solutions in our sample to be of the order of ~5-10% in our non-'validated' candidate samples. We demonstrate that Gaia is able to confirm and sometimes refine known orbital companion orbits as well as identify new candidates, providing us with a positive outlook of the expected harvest from the full mission data in future data releases.

==> DPACP-176_ Astrometric non-single stars processing with Markov Chain Monte Carlo and Genetic Algorithms/acronyms.tex <==
\section{Acronyms}\label{sec:acronyms}
{\small
\begin{tabular}{ll}
\hline\hline
\textbf{Acronym}  &  \textbf{Description}  \\ 
%2MASS & Two-Micron All Sky Survey \\
ADQL&Astronomical Data Query Language \\
%AGB&Asymptotic Giant Branch (star) \\
AL & ALong scan (direction) \\
AC & ACross scan (direction) \\
%AP & Astrophysical Parameters \\
%BH & Black hole \\
%BP & Gaia Blue Photometer \\
%CMD & Colour Magnitude Diagram \\
%DoF&Degree(s) of Freedom \\
DACE & \href{https://dace.unige.ch/dashboard/}{Data and Analysis Center for Exoplanets} \\
DE-MCMC & Differential Evolution Markov Chain Monte Carlo \\ %(Sect.~\ref{sec:method_mcmc}) \\
DPAC & Data Processing and Analysis Consortium \\
DR1 & \href{https://www.cosmos.esa.int/web/gaia/data-release-1}{Gaia Data Release 1} \\
DR2 & \href{https://www.cosmos.esa.int/web/gaia/data-release-2}{Gaia Data Release 2}\\
EDR3 & \href{https://www.cosmos.esa.int/web/gaia/early-data-release-3}{Gaia Early Data Release 3} \\
DR3 & \href{https://www.cosmos.esa.int/web/gaia/data-release-3}{Gaia Data Release 3} \\
%EB&Eclipsing Binary \\
%FLAME & Final Luminosity Age Mass Estimator \\
%FWHM&Full Width at Half-Maximum \\
GA & Genetic Algorithm \\ %(Sect.~\ref{sec:method_ga}) \\
%GALEX&GALaxy Evolution eXplorer \\
%GoF & Goodness of Fit \\
%GSPPhot&Generalised Stellar Parametriser PHOTometry \\
%GSPSpec&Generalised Stellar Parametriser SPECtroscopy \\
%GUCD & Gaia Ultra-cool Dwarf\\
%HealPix & Hierarchical Equal Area isoLatitude Pixelisation \\
%HPM & High Proper Motion \\
%HRD & Hertzsprung-Russell diagram\\
%IMF&Initial Mass Function \\
%LMC&Large Magellanic Cloud \\
%LPV & Long Period Variables \\
%LSF & Line Spread Function (one dimensional) \\
%MAD & Median Absolute Deviation \\
%MS&Main Sequence (star) \\
%NLS & Non linear spectro \\
%NS & Neutron star \\
NSS&Non-Single Star \\
%PMa&proper motion anomaly \\
%PSF & Point Spread Function (two dimensional) \\
%RGB&Red Giant Branch (star) \\
%RMS&Root-Mean-Square \\
%RP & Gaia Red Photometer \\
%RUWE&Re-normalised unit-weight error \\
%RV & Radial Velocity \\
%RVS&Radial Velocity Spectrometer \\
%SB & Spectroscopic Binary  \\
%SB2&Double-lined Spectroscopic Binary \\
%SNR & Signal to Noise ratio (also denoted SN and S/N)\\
%TBO & Two body orbits \\
%UCD&Ultra cool dwarf (star) \\
%UV&UltraViolet \\
%VIMF & variable-induced movers fixed \\
%WD & White dwarf\\
\hline
\end{tabular} 
}
